Low-Resolution Spectroscopy of Gamma-ray Burst Optical Afterglows: Biases in the Swift Sample and Characterization of the Absorbers

(Abridged). We present a sample of 77 optical afterglows (OAs) of Swift detected GRBs for which spectroscopic follow-up observations have been secured. We provide linelists and equivalent widths for all detected lines redward of Ly-alpha. We discuss to what extent the current sample of Swift bursts with OA spectroscopy is a biased subsample of all Swift detected GRBs. For that purpose we define an X-ray selected sample of Swift bursts with optimal conditions for ground-based follow up from the period March 2005 to September 2008; 146 bursts fulfill our sample criteria. We derive the redshift distribution for this sample and conclude that less than 19% of Swift bursts are at z>7. We compare the high energy properties for three sub-samples of bursts in the sample: i) bursts with redshifts measured from OA spectroscopy, ii) bursts with detected OA, but no OA-based redshift, and iii) bursts with no detection of the OA. The bursts in group i) have significantly less excess X-ray absorption than bursts in the other two groups. In addition, the fraction of dark bursts is 14% in group i), 38% in group ii) and > 39% in group iii). From this we conclude that the sample of GRBs with OA spectroscopy is not representative for all Swift bursts, most likely due to a bias against the most dusty sight-lines. Finally, we characterize GRB absorption systems as a class and compare them to QSO absorption systems, in particular DLAs. On average GRB absorbers are characterized by significantly stronger EWs for HI as well as for both low and high ionization metal lines than what is seen in intervening QSO absorbers. Based on the z>2 bursts in the sample we place a 95% confidence upper limit of 7.5% on the mean escape fraction of ionizing photons from star-forming galaxies.

==> author.tex <==
J. P. U. Fynbo,
P. Jakobsson,
J. X. Prochaska,
D. Malesani,
C. Ledoux,
A. de Ugarte Postigo,  
M. Nardini,
P. M. Vreeswijk,
K. Wiersema,
J. Hjorth,
J. Sollerman8,
H.-W. Chen,
C. C. Th\"one, 
G. Bj\"ornsson,
J. S. Bloom,
A. Castro-Tirado,
L. Christensen,
A. De Cia,
A. S. Fruchter,
J. U. Gorosabel,
J. F. Graham,
A. O. Jaunsen,
B. L. Jensen,
D. A. Kann,
C. Kouveliotou,
A. Levan,
J. Maund,
N. Masetti,
B. Milvang-Jensen,
E. Palazzi,
D. A. Perley,
E. Pian,
E. Rol,
P. Schady,
R. Starling,
N. Tanvir,
D. J. Watson,
D. Xu,
T. Augusteijn,
F. Grundahl,
J. Telting,
P.-O. Quirion

